Renaissance Robot: Optimal Transport Policy Fusion for Learning Diverse Skills

Deep reinforcement learning (RL) is a promising approach to solving complex robotics problems. However, the process of learning through trial-and-error interactions is often highly time-consuming, despite recent advancements in RL algorithms. Additionally, the success of RL is critically dependent on how well the reward-shaping function suits the task, which is also time-consuming to design. As agents trained on a variety of robotics problems continue to proliferate, the ability to reuse their valuable learning for new domains becomes increasingly significant. In this paper, we propose a post-hoc technique for policy fusion using Optimal Transport theory as a robust means of consolidating the knowledge of multiple agents that have been trained on distinct scenarios. We further demonstrate that this provides an improved weights initialisation of the neural network policy for learning new tasks, requiring less time and computational resources than either retraining the parent policies or training a new policy from scratch. Ultimately, our results on diverse agents commonly used in deep RL show that specialised knowledge can be unified into a "Renaissance agent", allowing for quicker learning of new skills.

==> background.tex <==
While there are many techniques for data fusion, fewer exist for model fusion. This is because it is more difficult to determine how and what to fuse for neural networks. The following works discussed in this section explain current approaches to combining the knowledge of multiple models, some of which have already been applied to RL policies. However, none of these approaches are viable as a computationally efficient way to achieve a single fused result that is capable of learning new and diverse skills, which is the aim of this paper.

\subsection{Ensembling}
Models have traditionally been combined via ensembling \cite{ensembling1,ensembling2, ensembling3}, whereby each model operates as an independent entity and only the results are synthesised (e.g. by majority prediction). This requires all models to be running concurrently, which is computationally expensive. Moreover, it does not actually aggregate each model's distinct capabilities, since decision making occurs separately. Hence, it is not suitable for adapting to customised tasks, especially when the learned behaviours of the parent models differ significantly.

\subsection{Distillation}
Distillation \cite{distillation1, distillation2, distillation3} is a technique that results in a single model, which is achieved by transferring knowledge from a larger teacher network (typically more expensive to train) to a smaller student network. However, distillation is often just as computationally expensive as training the student network from scratch, and often requires additional hyper-parameter tuning for the transfer process to be effective. It also requires sharing of training data between the teacher and student networks, which is often impractical in real-world scenarios. Another approach to distillation \cite{distillation_gan} proposes using a Generative Adversarial Network (GAN) \cite{gan} so that the student network is forced to mimic the teacher network. Yet, this still does not reduce the computational burden, nor does it provide a principled way to unify the ``intelligence" of different models.

\subsection{Network Fusion}
Network fusion methods have also been proposed, allowing for two parent models to be merged into a new child model, without the need for retraining. One such method involves using Elastic Weight Consolidation to construct an assignment problem based on the Hessian matrices of the two parent networks \cite{network_fusion1, network_fusion2, network_fusion3}. Whilst this does yield a combined model, it does not perform empirically better than naive averaging. Additionally, this method only works when all the weights of the parent networks are already very similar (e.g. by sharing a large portion of training history), since it relies on local Stochastic Gradient Descent (SGD). Thus, it is not generic enough for real-world applications, which likely require fusion of two parent models that have been built independently.

More recently, alignment-based methods have been considered, which match neurons between the parent networks before attempting to fuse them. ``Neural matching" is performed under a Bayesian non-parametric framework, with a specific focus on federated learning \cite{alignment1, alignment2}. In this framework, the number of parameters required grows with the size of the data, so it is infeasible for fusing large models. Nevertheless, since it is designed mainly for federated learning, it is not directly usable in general applications. More recently, others have used OT theory to fuse neural network models \cite{model_fusion_via_ot}, although this has not yet been applied to RL.

